Tracking the Evolution of Static Code Warnings: the State-of-the-Art and a Better Approach

Static bug detection tools help developers detect problems in the code, including bad programming practices and potential defects. Recent efforts to integrate static bug detectors in modern software development workflows, such as in code review and continuous integration, are shown to better motivate developers to fix the reported warnings on the fly. A proper mechanism to track the evolution of the reported warnings can better support such integration. Moreover, tracking the static code warnings will benefit many downstream software engineering tasks, such as learning the fix patterns for automated program repair, and learning which warnings are of more interest, so they can be prioritized automatically. In addition, the utilization of tracking tools enables developers to concentrate on the most recent and actionable static warnings rather than being overwhelmed by the thousands of warnings from the entire project. This, in turn, enhances the utilization of static analysis tools. Hence, precisely tracking the warnings by static bug detectors is critical to improving the utilization of static bug detectors further.

==> Makefile <==

default: paper
	@echo '****************************************************************'
	@echo '**************** Did you spell-check the paper? ****************'
	@echo '****************************************************************'
coall:
	co RCS/*

ciall:
	ci -u *.tex
	ci -u *.eps

bib: paper.bbl

paper.bbl: *.tex paper.bib
	latex paper
	bibtex paper
	latex paper

paper.ps: paper.dvi
	dvips -P cmz paper.dvi -o paper.ps -t letter

paper.dvi: *.tex paper.bbl
	latex paper
	latex paper

paper.pdf: *.tex
	pdflatex paper
	pdflatex paper
mpost:
	mpost -tex=latex overview.mp

paper: *.tex
	pdflatex paper
	bibtex paper
	pdflatex paper
	#pdf2ps paper.pdf paper.ps

patent: patent.tex
	pdflatex patent

cover: cover.tex
	pdflatex cover
	bibtex paper
	pdflatex cover
	pdflatex cover
	pdflatex cover2

purge:
	rm -f   *.aux \
                *.bbl \
                *.blg \
                *.dvi \
                *.log \
                *.toc \
                paper.ps \
		overview.mps\
		paper.pdf

clean:
	rm -f   *.aux \
                *.bbl \
                *.blg \
                *.dvi \
                *.log \
                *.toc \
                paper.ps



